Joint Modelling of Astrophysical Systematics for Cosmology with LSST Cosmic Shear

We present a novel framework for jointly modelling the weak lensing source galaxy redshift distribution and the intrinsic alignment of galaxies via a shared luminosity function (LF). Considering this framework within the context of a Rubin Observatory's Legacy Survey of Space and Time (LSST) Year 1 and Year 10 cosmic shear analysis, we first demonstrate the substantial impact of the LF on both source galaxy redshift distributions and the intrinsic alignment contamination. We establish how the individual parameters of a Schechter LF model impact the redshift distribution of a magnitude-limited sample, and we demonstrate the effect of marginalising over the LF parameters as incorporated in the intrinsic alignment modelling of a standard cosmic shear analysis set-up. We forecast the impact of our joint modelling framework on cosmological parameter constraints. Our preliminary results are promising, indicating that this framework can yield cosmological constraints consistent with those expected from standard analyses, enhanced by the flexibility of not fixing LF parameters. We plan to further validate these findings with comprehensive Markov chain Monte Carlo simulations to robustly quantify bias avoidance and underscore the framework's efficacy. Taking advantage of our forecasting results and the parameter degeneracies, we identify the specific impact of the shape of the LF of source galaxies on the cosmic shear data vector. We also discuss the potential of this method in providing a way to model generic selection functions in redshift distribution estimation, as well as its possibilities for extension to a 3x2pt analysis, particularly with respect to incorporating galaxy bias in this luminosity-function-based framework. Although we consider the context of LSST cosmic shear in this work, the proposed joint modelling framework is generically applicable to weak lensing surveys.

==> figures/corner_jmas_cosmolf_crop.tex <==
\begin{figure*}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[height=0.27\textheight]{figures/fig_files/corner_jmas_y1_cosmoialf_crop.pdf}
\caption{Cosmological and LF parameters, LSST Y1} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[height=0.27\textheight]{figures/fig_files/corner_jmas_y10_cosmoialf_crop.pdf}
\caption{Cosmological and LF parameters, LSST Y10} \label{fig:b}
\end{subfigure}
\medskip
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[height=0.27\textheight]{figures/fig_files/corner_jmas_ialf_y1_crop.pdf}
\caption{IA and LF parameters, LSST Y1} \label{fig:c}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[height=0.27\textheight]{figures/fig_files/corner_jmas_ialf_y10_crop.pdf}
\caption{IA and LF parameters, LSST Y10} \label{fig:d}
\end{subfigure}
\medskip
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[height=0.27\textheight]{figures/fig_files/corner_jmas_lf_y1.pdf}
\caption{LF parameters, LSST Y1} \label{fig:e}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[height=0.27\textheight]{figures/fig_files/corner_jmas_lf_y10.pdf}
\caption{LF parameters, LSST Y10} \label{fig:f}
\end{subfigure}
\caption{\textit{Segments of the Fisher matrix marginalized contours for JMAS analysis across forecasting years.}
This figure showcases six plots illustrating the correlations between parameters: the top row details the interactions between cosmological and LF parameters; the middle row explores the correlations between IA and LF parameters; and the bottom row examines the LF parameters' interrelations.
Green contours (left column) represent forecasts for LSST Year 1 (Y1), while blue contours (right column) depict Year 10 (Y10) forecasts, demonstrating the evolution of parameter sensitivities over time.} \label{fig:all_correlations_minipage}
\end{figure*}

==> figures/jmas_srd_cls_relative_difference.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.5]
{figures/fig_files/data_vectors_srd_jmas_ratios.pdf}
    \caption{Relative difference of the joint modelling and standard analysis angular power spectra for forecasting Years 1 and 10.
    We present the ratios  for each correlation, with Year 1 shown in green and Year 10 in blue.
    The key emphasis here is not the differentiation between individual correlations but to highlight that all observed deviations remain below the 15\% threshold. 
    This result is a critical aspect of our validation process, confirming the effectiveness and accuracy of our joint modeling method.
    By consistently aligning with the SRD benchmarks and maintaining acceptable deviation limits across both forecasting years, this analysis plays a pivotal role in validating our joint modeling approach, showcasing its robustness and reliability in the face of varying forecasting scenarios.}
\label{fig:datavectors_relative_difference}
\end{figure*}
